The 3rd Reactive Synthesis Competition (SYNTCOMP 2016): Benchmarks, Participants & Results

We report on the benchmarks, participants and results of the third reactive synthesis competition(SYNTCOMP 2016). The benchmark library of SYNTCOMP 2016 has been extended to benchmarks in the new LTL-based temporal logic synthesis format (TLSF), and 2 new sets of benchmarks for the existing AIGER-based format for safety specifications. The participants of SYNTCOMP 2016 can be separated according to these two classes of specifications, and we give an overview of the 6 tools that entered the competition in the AIGER-based track, and the 3 participants that entered the TLSF-based track. We briefly describe the benchmark selection, evaluation scheme and the experimental setup of SYNTCOMP 2016. Finally, we present and analyze the results of our experimental evaluation, including a comparison to participants of previous competitions and a legacy tool.

==> eptcsdata.tex <==
\providecommand{\firstpage}{149}
\providecommand{\publicationstatus}{Dimitrova, Piskac (Eds.): Fifth Workshop on\\ 
Synthesis (SYNT 2016)\\
EPTCS 229, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.229.12}{10.4204/EPTCS.229.12}}
\pdfoutput=1
\usepackage{ifthen}
\providecommand{\eptcs}{{\sl Electronic Proceedings in Theoretical Computer Science}}
\providecommand{\opa}{, Open Publishing Association}
\providecommand{\finishreference}[6]{#1 #2#3, pp. #4--#5, \doi{10.4204/EPTCS.#2.#6}}
\providecommand{\thisvolume}[2][\eptcs]{%
 \ifthenelse{\equal{#2}{5}}{\finishreference{#1}{229}{\opa}{133}{148}{11}}{%
 \ifthenelse{\equal{#2}{1}}{\finishreference{#1}{229}{\opa}{112}{132}{10}}{%
 this volume of #1\opa}}}

